A Unified Framework for Light Spanners

Seminal works on light spanners over the years have provided spanners with optimal lightness in various graph classes, such as general graphs, Euclidean spanners, and minor-free graphs. Three shortcomings of previous works on light spanners are: (i) The runtimes of these constructions are almost always sub-optimal and usually far from optimal. (ii) These constructions are optimal in the standard and crude sense but not in a refined sense that takes into account a wider range of involved parameters. (iii) The techniques are ad hoc per graph class and thus can't be applied broadly. This work aims at addressing these shortcomings by presenting a unified framework of light spanners in a variety of graph classes. Informally, the framework boils down to a transformation from sparse spanners to light spanners; since the state-of-the-art for sparse spanners is much more advanced than that for light spanners, such a transformation is powerful. First, we apply our framework to design fast constructions with optimal lightness for several graph classes. Second, we apply our framework to achieve more refined optimality bounds for several graph classes, i.e., the bounds remain optimal when taking into account a wider range of involved parameters, most notably $\epsilon$. Our new constructions are significantly better than the state-of-the-art for every examined graph class.

==> ACTapp.tex <==
\section{The Algebraic Computation Tree Model} \label{algapp}
 In this appendix we give a brief description of the {\em algebraic computation tree (ACT)} model. 
 (Refer to \cite{BenOr83} and Chapter 3 in the book \cite{NS07} for a more detailed description.)
%(Refer to \cite{BenOr83,NS07} for a more detailed description.)

An ACT is a binary computation tree where each leaf is associated with an output and each internal node is either (\emph{i}) labeled with a variable $f_x$ determined by $f_x = a_1\circ a_2$ or $f_x = \sqrt{a_1}$ where $\circ \in \{+,-,\times,\div\}$ and each $a_i$, $i \in \{1,2\}$, is either a value of a proper ancestor of $x$, an input element or a constant in $\mathbb{R}$, or (\emph{ii}) labeled with a comparison $a \bowtie 0$, where $a$ is either a value of a proper ancestor of $x$, or an input element, and the left (resp. right) child is labeled with ``$\le$''  (resp. ``$>$''). An ACT tree $T$ corresponds to an algorithm $\mathcal{A}_T$, which traverses a path down the tree starting at the root and either (\emph{i}) evaluates $f_x$ if the node has one child, or (\emph{ii}) selects left or right child depending on the outcome of the comparison. When $\mathcal{A}_T$ reaches the leaf, it evaluates the expression by replacing all the variables with the input values and terminates. It is required that no input lead to undefined behavior, such as division by 0, or taking a square root of a negative number; furthermore, for each leaf $w$ there should be an input on which $\mathcal{A}_T$ terminates in $w$. 
A problem $\mathcal{P}$ is solvable in the ACT model if there exists an ACT tree $T$ such that for any valid input for $\mathcal{P}$, $\mathcal{A}_T$ returns the value of $\mathcal{P}$ on that input. 

The ACT model is particularly convenient for proving lower bounds, as it encompasses and represents explicitly all possible execution paths of an algorithm. For most algorithmic purposes, one can alternatively consider the real RAM model; one can prove an equivalence between the two models, which holds up to some subtle issues of uniformity that lie outside the scope of the current paper.


\section{Proof of \Cref{lm:Clustering2-Step5B1E}}\label{app:Clustering-5BProofE}


We follow the same construction in~\cite{LS19}.  We color the contracted nodes of  $\Pbar$ by black color, and other nodes by white color. Let $\bar{W}$ be the set of black nodes of $\Pbar$. Let $\me_{white}$ be the set of edges between two white nodes of $\Pbar$, called white edges. We will orient edges in $\me_i^{\take -}(\Pbar)\setminus  \me_{white}$ as out-going from their black endpoints. Thus, in what follows, we only focus on  orienting white edges. 


Let $\Ptilde^{\uncontract}$ be obtained from $\Pbar$ by uncontracting contracted nodes. Let $\tilde{W}$ be the set of nodes in $\Ptilde^{\uncontract}$ that are in contracted nodes of $\Pbar$. We color nodes in $\tilde{W}$ by black color, and other nodes by white color.  Due to a special structure of contracted nodes (as shown in \Cref{lm:Clustering2-Step2T2}), we can show that the potential change of a subgraph $\mx$ to be constructed is proportional to the number black nodes it has. Thus, the remaining challenge is to relate the potential change with the number of white edges incident to $\mx$. This is basically accomplished in the construction of \dblind\cite{LS19}; for completeness, we include a proof below.


\begin{lemma}[Lemma 6.17~\cite{LS19}]\label{lm:Clustering-White} We can construct a set of subgraphs $\mathbb{C}_5(\Pbar)$ such that: 	
	\begin{enumerate}
		\item[(1)]  Subgraphs in $\mathbb{C}_5(\Pbar)$ contain every node in $\Ptilde^{\uncontract}$.
		\item[(2)] For every subgraph $\mx\in \mathbb{C}_5(\Pbar)$, $\zeta L_i \leq \adm(\mx)\leq 5L_i$. Furthermore, $\mx$ is a subtree of $\Ptilde^{\uncontract}$ and some edges in  $\me_{white}$  whose both endpoints are in $\mx$.
		\item[(3)]  There is an orientation of edges in $\me_{white}$  
		such that, for any subgraph $\mx \in  \mathbb{C}_5(\Pbar)$,  if the total number of out-going edges incident to nodes in $\mx$ is $t$ for any $t\geq 0$, then:
		\begin{equation}\label{eq:Step5BpotentialWhite}
			\Delta^+_{i+1}(\mx) =  \Omega(t\eps + |\mv(\mx)\cap \tilde{W}|)\eps L_i
		\end{equation}
	\end{enumerate}
\end{lemma}

We now show that \Cref{lm:Clustering-White} implies \Cref{lm:Clustering2-Step5B1E}.

\begin{proof}[Proof of \Cref{lm:Clustering2-Step5B1E}] Let  $\mathbb{C}_5(\Pbar)$  be the set of subgraphs constructed by \Cref{lm:Clustering-White}. Items (1) and (2) of \Cref{lm:Clustering2-Step5B1E} follows directly from Items (1) and (2) of \Cref{lm:Clustering-White}. Thus, it remains to show Item (3).
	
	We orient edges of $\me_i^{\take -}(\Pbar)$ as follows. Edges in $  \me_{white}$ are oriented following \Cref{lm:Clustering-White}. For each edge in  $\me_i^{\take -}(\Pbar)\setminus  \me_{white}$, we orient it as out-going from (arbitrary) one of its black endpoint(s); there must exist at least one black endpoint by the definition of $\me_{white}$. 
	
	Let $t$ be the number of out-going edges in $\me_i^{\take -}(\Pbar)$ incident  to nodes in $\mx$. Let $t_1$ be the number of out-going edges in $\me_{white}$ incident to $\mx$, and $t_2 =  t-t_1$. By the construction in Step 1 (\Cref{lm:Clustering2-Step1T2}), every node in $\mx$ is incident to at most $\frac{2g}{\zeta \eps} = O(1/\eps)$ edges in  $\me_i$. Thus, $t_2\leq O(1/\eps) |\mv(\mx)\cap \tilde{W}|$. That is, $ |\mv(\mx)\cap \tilde{W}| = \Omega(t_2\eps)$. Thus, by \Cref{eq:Step5BpotentialWhite}, we have:
	\begin{equation*}
		\Delta^+_{i+1}(\mx) =  \Omega(t_1\eps + t_2\eps)\eps L_i =  \Omega(t)\eps^2L_i
	\end{equation*}
	as claimed.
	\qed
\end{proof}



We now focus on proving \Cref{lm:Clustering-White}. There are two main steps in the construction. 

\paragraph{Step 1: tiny clusters.~} We greedily break $\Pbar$ into subpaths of augmented diameter at least $\zeta L_i$ and at most $3\zeta L_i$. This is possible since each node has weight at most $\zeta L_i$ due to the construction in Step 2 (\Cref{lm:Clustering2-Step2T2}) and each edge has weight at most $\eps L_i \leq \zeta L_i$ when $\eps \leq \zeta$. Each subpath of $\Pbar$ is called a tiny cluster.  Let $\mathbb{C}_{tiny}$ be the set of all tiny clusters.

Since $3\zeta L_i < L_i/(2)$ (as $\zeta = 1/250$), there is no edge in $\me_i^{\take -}(\Pbar)$ whose both endpoints are in the same tiny cluster.  However, there may be parallel edges: two edges of $\me_{white}$ connecting the same two tiny clusters.



Let $\widehat{P}$ be obtained from $\Pbar$ by contracting each tiny cluster in a single \emph{supernode}. We abuse notation here by viewing  $\me_{white}$ as edges between contracted nodes in $\widehat{P}$.  Given a supernode $\hat{\nu}\in \widehat{P}$, we say that an edge  $\hat{\mbe}\in \me_{white}$ \emph{shadows} $\hat{\nu}$ if  $\hat{\nu}$ lies on the subpath of  $\widehat{P}$  between two endpoints of $\hat{\mbe}$. Note that edges incident to $\hat{\nu}$ shadow  $\hat{\nu}$  by definition. 


\paragraph{Step 2: constructing $ \mathbb{C}_5(\Pbar)$ and orient edges.~}  We iteratively construct a set of subgraphs $ \widehat{\mathbb{C}}_5$ from $\widehat{P}$ and $\me_{white}$, orient edges of $\me_{white}$ and mark contracted nodes of $\widehat{P}$ along the way.  Let  $\hat{\nu} \in \widehat{P}$ be an unmarked supernode  incident to a maximum number of \emph{unoriented edges} in $\me_{white}$. Let $\me_{white}(\hat{\nu})\subseteq \me_{white}$ be the set of unoriented edges shadowing $\hat{\nu}$; $\me_{white}(\hat{\nu})$ could be empty. Let  $\widehat{Q}$ be the minimal subpath of  $\widehat{P}$ that contains $\hat{\nu}$ and the endpoints of every edge in $\me_{white}(\hat{\nu})$. (If $\me_{white}(\hat{\nu}) = \emp$ then $\widehat{Q}$ contains a single node $\hat{\nu}$.) We refer to $\hat{\nu}$ as\emph{ the center} of  $\widehat{Q}$. We add the subgraph $\widehat{Q} \cup \me_{white}(\hat{\nu})$ to $ \widehat{\mathbb{C}}_5$. (See \Cref{fig:clustering-tiny}.) Next, we orient unoriented edges of  $\me_{white}$ incident to contracted nodes in $\widehat{Q}$ as out-going from $\widehat{Q}$. We then repeat this step until there is no unmarked supernode in $\widehat{P}$. Finally, we construct  $\mathbb{C}_5(\Pbar)$ by uncontracting each supernode  in $ \widehat{\mathbb{C}}_5$ twice; the first uncontraction gives a subbgraph of $\Pbar\cup \me_{white}$ and the second uncontraction gives a subgraph of $\Ptilde^{\uncontract}\cup \me_{white}$.  This completes the construction of  $\mathbb{C}_5(\Pbar)$ in \Cref{lm:Clustering-White}.

\begin{claim}\label{clm:hatP-structure} During the construction of Step 2,  if  we remove marked supernodes from $\widehat{P}$, then there is no edge in $\me_{white}$ connecting two nodes in two different connected components. 
\end{claim}
\begin{proof} We assume inductively that the claim is true before the removal of  $\widehat{Q}$ in Step 2. Thus,   $\widehat{Q}$  is a subpath of a connected component, say $\widehat{P}_1$,  of $\widehat{P}$ induced by unmakred contracted nodes. Marking contracted nodes of $\widehat{Q}$  could break  $\widehat{P}_1$ into two subpaths say  $\widehat{P}_2$ and  $\widehat{P}_3$, of unmarked contracted nodes. However, any edge of $\me_{white}$ between $\widehat{P}_2$ and  $\widehat{P}_3$ must shadow the center $\hat{\nu}$ of $\widehat{Q}$. That is, there is an edge in $\me_{white}(\hat{\nu})$ whose endpoints are not in $\widehat{Q}$, contradicting the construction in Step 2. \qed
\end{proof}



\begin{figure}[htb]
	\center{\includegraphics[width=0.9\textwidth]{figs/clustering-tiny}}
	\caption{Rectangular nodes are tiny clusters. Every unoriented edge incident to contracted nodes of $\widehat{Q}$ will be oriented as out-going from $\widehat{Q}$ (except those with both endpoints in  $\widehat{Q}$, which will be oriented arbitrarily). Solid edges are in $\me_{white}(\hat{\nu})$ whose both endpoints are white nodes.}
	\label{fig:clustering-tiny}
\end{figure} 


We now focus on proving the properties of $\mathbb{C}_5(\Pbar)$  claimed in \Cref{lm:Clustering-White}. Item (1) follows directly from the construction. Item (2) follows from the following claim.

\begin{claim} \label{clm:edm-IV}
	$\zeta L_i \leq \adm(\widehat{Q}) \leq 5L_i$.
\end{claim}
\begin{proof}
	The lower bound of $ \adm(\widehat{Q}) $ follows directly from the construction. For each edge $\hat{\mbe} = (\dbar{\alpha},\dbar{\beta})$  with both endpoints in $ \adm(\widehat{Q})$, we claim that \begin{equation}\label{eq:diam-shadow}
		\adm(\widehat{Q}[\dbar{\alpha},\dbar{\beta}]) \leq 2(1+3\zeta)L_i
	\end{equation}
	Let $\Qbar$ be obtained from $\widehat{Q}$ by uncontracting tiny clusters; $\Qbar$ is a path.  Let  $\bar{\alpha}$ and $\bar{\beta}$ be endpoints of $\hat{\mbe}$ on $\Qbar$; $\bar{\alpha}$ and $\bar{\beta}$  are nodes in the subpaths constituting tiny clusters  $\dbar{\alpha}$ and $\dbar{\beta}$, respectively. By definition  of $\bar{\me}_i^{close}$ in \Cref{eq:Ebar-farclose},  two intervals $\overline{\mathcal{I}}(\bar{\alpha})$ and $\overline{\mathcal{I}}(\bar{\beta})$ has $\overline{\mathcal{I}}(\bar{\alpha})\cap \overline{\mathcal{I}}(\bar{\beta}) \not=\emptyset$. By definition, each interval, say $\overline{\mathcal{I}}(\bar{\alpha})$, includes all contracted nodes within augmented distance $(1-\psi)L_i \leq L_i$ from $\bar{\alpha}$. This implies $\widehat{Q}[\bar{\alpha}, \bar{\beta}]\leq 2L_i$; thus Equation~\eqref{eq:diam-shadow} holds.  (An extra term $6\zeta L_i$ in \Cref{eq:diam-shadow}  is the upper bound on the sum of augmented diameters of $\dbar{\alpha}$ and $ \dbar{\beta}$.)
	
	
	Let $\dbar\nu_0, \dbar\mu_0$ be the two tiny clusters that are endpoints of $\widehat{Q}$. Let $\hat{\mbe}_1 = (\dbar{\nu}_0, \dbar{\nu}_1)$ and $\hat{\mbe}_2 = (\dbar{\mu}_0, \dbar{\mu}_1)$	be two edges shadowing $\dbar{\nu}$, the center of $\widehat{Q}$. Two edges $\hat{\mbe}_1$ and $\hat{\mbe}_2$ exist by the minimality of $\widehat{Q}$. Then:
	\begin{equation*}
		\adm(\widehat{Q}) \leq \adm(\widehat{Q}[\dbar{\nu}_0, \dbar{\nu}_1]) + \adm(\widehat{Q}[\dbar{\mu}_0, \dbar{\mu}_1]) \stackrel{\text{Eq.~\eqref{eq:diam-shadow}}}{\leq} 4(1+3\zeta)L_i  < 5L_i
	\end{equation*}
	as $\zeta = \frac{1}{250}$.\QED
\end{proof}

We now show Item (3) of \Cref{lm:Clustering-White}.  Observe that by construction, $\widehat{Q}$ consists of a path of at most $\frac{5}{\zeta} = O(1)$ tiny clusters since $\adm(\hat{Q})\leq 5L_i$ while each tiny cluster has an augmented diameter at least $\zeta L_i$ . Let $\Qbar$ be obtained from $\widehat{Q}$  by uncontracting tiny clusters, and $\mathcal{Q}$ be obtained from $\Qbar$ by uncontracting contracted nodes. (Note by construction that $\Qbar$  is a path.) Let $\md$ be the diameter path of $\mq$; it could be that $\md$ contains edges in $\me_{white}(\hat{\nu})$.


Let $\widehat{Q}^-$ be obtained from $\widehat{Q}$ by removing all edges in $\me_{white}(\hat{\nu})$; $\hat{\nu}$ is the center of $\widehat{Q}$. Let $\Qbar^{-}$ and $\mq^-$ be obtained from $\Qbar$ and $\mq$ by removing all edges in $\me_{white}(\hat{\nu})$, respectively.  Let $\md^-$ be the shortest path in $\mq^-$ (w.r.t both edge and node weights) between $\md$'s endpoints. (See Figure~\ref{fig:uncontract-tiny}).  Observe that:


\begin{observation}\label{obs:Dminus-vs-AdmX}
	$\adm(\md^-)\geq \adm(\mq)$.
\end{observation}
\begin{proof}
	We have $\adm(\md^-) \geq \adm(\md) = \adm(\mq)$.\qed.
\end{proof}
\begin{figure}[!ht]
	\centering
	\includegraphics[scale = 1.5]{figs/uncontract-tiny.pdf}
	\caption{\footnotesize{(a) A subgraph $\widehat{Q}$ formed in Step 5A; triangular blocks are tiny clusters. Solid blue edges are edges in $\me_{white}(\hat{\nu})$. (b) $\mq$ obtained by uncontracting tiny clusters and  contracted nodes. Diameter path $\md$ of $\mq$ is highlighted red; the path $\md^{-}$ is highlighted blue. Solid blue edges are in $\md$.}}
	\label{fig:uncontract-tiny}
\end{figure}


Let 	$\me_{white}({\widehat{Q}})$ be the set of edges in $\me_{white}$ incident to tiny clusters in $\widehat{Q}$.  By construction, $\dbar{\nu}$ is incident to the maximum number of edges in $ \me_{white}$ over every node in $\widehat{Q}$. (Note that $\widehat{Q}$ only has $O(1)$ tiny clusters.) This implies that:

\begin{observation}\label{obs:Incident-tiny}
	$|\me_{white}({\widehat{Q}})| = O(| \me_{white}(\dbar{\nu})|)$.
\end{observation}

We now define:
\begin{equation}\label{eq:PhiX}
	\Phi(\mq) = \sum_{\varphi \in \mv(\mq)}\omega(\varphi) + \sum_{\mbe \in \msttilde_i\cap \me(\mq)}w(\mbe)
\end{equation}
Observe by the definition that:
\begin{equation}\label{eq:Potential-vs-Phi}
	\begin{split}
		\Delta^+_{i+1}(\mq) &= \Delta_{i+1}(\mq) +  \sum_{\mbe \in \msttilde_i\cap \me(\mq)}w(\mbe)\\
		&= \sum_{\varphi \in \mv(\mq)}\omega(\varphi) - \adm(\mq) +  \sum_{\mbe \in \msttilde_i\cap \me(\mq)}w(\mbe)\\
		&= \Phi(\mq) - 		\adm(\mq) 
	\end{split}
\end{equation}

\begin{lemma}\label{lm:leftover-LS19} Let $\mu$ be node in $\md^-$ that is incident to $t \geq 1$ edges in  $\me_{white}(\dbar{\nu})$. Then  $\Delta^+_{i+1}(\mq)= \Omega(t\epsilon L_i)$.
\end{lemma}
\begin{proof} Let $\mz$ be the set other $t$ endpoints  of $t$ edges incident to $\mu$. If $|\mz \cap \md|\leq t/2$, then:
	\begin{equation*}
		\begin{split}
			\Delta^+_{i+1}(\mq) &= \Phi(\mq) - \adm(\mq) \stackrel{\mbox{Obs.~\ref{obs:Dminus-vs-AdmX}}}{\geq} \Phi(\mq) - \adm(\md^-)\\
			&\geq \adm(\mz\setminus \md) \stackrel{\mbox{Eq.~\eqref{eq:PhiX}}}{\geq} O(|\mz\setminus \md|\epsilon L_i) = \Omega(t\epsilon L_i),
		\end{split}
	\end{equation*}
	as claimed. 
	
	
	
	\begin{wrapfigure}{r}{0.45\textwidth}
		\vspace{-35pt}
		\begin{center}
			\includegraphics[width=0.45\textwidth]{figs/z-right}
		\end{center}
		\caption{\footnotesize{(a) blue edges are level-$i$ edges incident to $\mu$. (b) $\md_j$ obtained by replacing $\md_{j-1}[\mu,\alpha_{j}]$ by $\mp_j = (\mu,e,\alpha_{j})$.}}
		\vspace{-5pt}
		\label{fig:z-right}
	\end{wrapfigure}
	
	Herein, we assume that  $|\mz \cap \md|\geq t/2$. We can also assume~w.l.o.g. that at least $t/4$ nodes in $\mz$ that are to the right of $\mu$ on $\md^-$. (Note that $\md^-$ contains only $\widetilde{\mst}_i$ edges.) Let $\mz_{right} = \{\alpha_1,\ldots, \alpha_s\}$, $s \geq t/4$,  be the set of nodes to the right of $\mu$, and such that $\alpha_{j-1}\in \md^{-}[\mu, \alpha_{j}]$ for any $j\in [2,s]$ (see Figure~\ref{fig:z-right}(a)). Let $\mbe_j = (\mu,\alpha_j)$ be the edge in $\me_{white}(\dbar{\nu})$ between $\mu$ and $\alpha_j$, $j \in [2]$. By construction, $\Qbar$ is  a path. Note that edges in $\me_{white}$ have white nodes as endpoints, which by definition, are uncontracted nodes in $\Qbar$, and hence $\mu$ and $\alpha_j$ are uncontracted nodes. That is, $\mu = \bar{\mu}$ and $\alpha_j = \bar{\alpha}_j$.  
	
	Let $\md_0 = \md^-$ and we define $\md_j$ for each $j \in [1,s]$ as follows: $\md_{j}$ is obtained from $\md_{j-1}$ by replacing the subpath $\md_{j-1}[\mu, \alpha_{j}]$ by path $\mp_{j} \stackrel{\mbox{def.}}{=} (\mu, \mbe_j, \alpha_{j})$ which has only one edge $\mbe_j$ (see Figure~\ref{fig:z-right}(b)). 
	
	\begin{claim}\label{clm:dj-vs-dj1}
		$\adm(\md_j) \leq \adm(\md_{j-1}) + \epsilon g L_i$.
	\end{claim}
	\begin{proof}
		We have: 
		
		\begin{equation*}
			\begin{split}
				\adm(\md_{j-1}) - \adm(\md_j) &= w(\md_{j-1}[\nu,\mu]) - \omega(\mp_j) \geq  d_{\mathcal{H}_i}(\nu,\mu) - \omega(\mp_j) \\
				&\geq 6g\epsilon  \cdot \omega(\mbe_j)  - \omega(\nu) - \omega(\mu) \qquad \mbox{(by \Cref{obs:greedy-HiE})} \\
				&\geq 6g\epsilon L_i/2 - 2g\epsilon L_i = g\epsilon L_i,
			\end{split}
		\end{equation*}
		as claimed.\qed
	\end{proof}
	
	
	By Claim~\ref{clm:dj-vs-dj1}, we have:
	\begin{equation}\label{eq:mds-vs-mdM}
		\adm(\md_s) ~\leq~ \adm(\md_0) + s\epsilon g L_i ~=~ \adm(\md^-) + s\epsilon g L_i.
	\end{equation}
	Since $\md_s$ and $\md$ has the same endpoint and $\md$ is a shortest path, $\adm(\md_s)\geq \adm(\md)$.  This implies:
	\begin{equation*}
		\begin{split}
			\Delta^+_{i+1}(\mq) &= \Phi(\mq) - \adm(\mq) =  \Phi(\mq) - \adm(\md)\\
			&\geq \Phi(\mq)  - \adm(\md_s) \geq \adm(\md^-) - \adm(\md_s)\\
			&\stackrel{\mbox{Eq.~\eqref{eq:mds-vs-mdM}}}{\geq} s\epsilon g L_i = \Omega(t\epsilon L_i),\qquad \mbox{since }s\geq t/4 
		\end{split}
	\end{equation*}
	as desired.\qed		
\end{proof}


\begin{lemma}\label{lm:H5}
	$\Delta^+_{i+1}(\mq) = \Omega(\eps^2)|\me_{white}(\widehat{Q})|L_i$.
\end{lemma}
\begin{proof}
	Suppose that $|\me_{white}(\dbar{\nu})| = \frac{t}{\epsilon}$ for some $t > 0$. By Observation~\ref{obs:Incident-tiny}, it holds that $|\me_{white}(\widehat{Q})| = O( \frac{t}{\epsilon})$. This implies:
	\begin{equation}\label{eq:Size-Etiny-X}
		t = \Omega(\eps)|\me_{white}(\widehat{Q})|
	\end{equation}
	
	Let $\overline{\mp}$ be the path of contracted nodes corresponding to tiny cluster $\dbar{\nu}$. Let $\mz$ be the set of uncontracted nodes of $\overline{\mp}$ that are incident to at least $\frac{t \zeta}{4g}$ edges in $\me_{white}(\hat{\nu})$. We claim that:
	\begin{claim}\label{clm:Size-Z}
		$|\mz|\geq \frac{t\zeta}{4g}$.
	\end{claim}
	\begin{proof}
		Let $\ma$ be the set of remaining uncontracted nodes in  $\overline{\mp}\setminus \mz$.  Then $|\ma|\leq \frac{\adm(\overline{\mp})}{\zeta L_{i-1}} = \frac{2g}{\zeta \epsilon}$ since $\adm(\overline{\mp})\leq gL_i$. Recall that each in $\mz$ is incident to at most $\frac{2g}{\epsilon}$ edges by the construction in Step 1 (\Cref{lm:Clustering2-Step1T2}).  Thus, we have:
		\begin{equation*}
			|\me_{white}(\dbar{\nu})| \leq |\mz|\frac{2g}{\zeta\epsilon} + \frac{t \zeta}{4g} |\ma|  < \frac{t\zeta}{4g} \cdot \frac{2g}{\zeta \eps} + \frac{t \zeta}{4g} \cdot \frac{2g}{\zeta \epsilon} = \frac{t}{\epsilon}
		\end{equation*}	
		This is a contradiction since $|\me_{white}(\dbar{\nu})| = \frac{t}{\epsilon}$.\qed
	\end{proof}
	We consider two cases:
	\begin{itemize}
		\item \textbf{Case 1:} $\mathcal{D}^- \cap \mz \not= \emptyset$.  By Lemma~\ref{lm:leftover-LS19}, $\Delta^+_{i+1}(\mq) = \Omega(\frac{t \zeta}{4g} \epsilon L_i) = \Omega(t \epsilon L_i)$ since every node in $\mz$ is incident to at least $\frac{t \zeta}{4g}$ edges in $\me_{white}(\hat{\nu})$. By Equation~\eqref{eq:Size-Etiny-X}, $\Delta^+_{i+1}(\mq) = \Omega(\epsilon^2) |\me_{white}(\widehat{Q})| L_i$.
		
		\item  \textbf{Case 1:} $\mathcal{D}^- \cap \mz = \emptyset$. Then, it holds that:
		\begin{equation*}
			\begin{split}
				\Delta^+_{i+1}(\mq) &= \Phi(\mq^-) - \adm(\mq) \stackrel{\mbox{Obs.~\ref{obs:Dminus-vs-AdmX}}}{\geq }\Phi(\mq^-) - \md^- \\
				&\geq~ \sum_{\varphi \in \mz} \omega(\varphi)  = \Omega(|\mz|\epsilon L_i) = \Omega(t\epsilon L_i)  =  \Omega(\epsilon^2) |\me_{white}(\widehat{Q})| L_i 
			\end{split}
		\end{equation*}
	\end{itemize} 
	In both cases,  the lemma holds. \qed
\end{proof}

We note that out-going edges of $\me_{white}$ incident to nodes in $\mathcal{Q}$ are $\me_{white}(\hat{Q})$. Thus, the following lemma implies  Item (3) of \Cref{lm:Clustering-White}. 

\begin{lemma} $	\Delta^+_{i+1}(\mq) =  \Omega(|\me_{white}(\hat{Q})|\eps + |\mv(\mq)\cap \tilde{W}|)\eps L_i$.
\end{lemma}
\begin{proof} We will show that:
	\begin{equation}\label{eq:blacknodes-C}
		\Delta^+_{i+1}(\mq) =  \Omega(|\mathcal{Q} \cap \tilde{W}|) \epsilon L_i
	\end{equation}
	The lemma then follows from \Cref{eq:blacknodes-C} and \Cref{lm:H5}.
	
	Let $\bar{\mu}$ be a black node in $\Qbar$; $\bar{\mu}\in \Qbar\cap \bar{W}$. Let $\mathcal{T}_{\bar{\mu}}$ be the subtree of $\msttilde_{i}$ corresponding to $\bar{\mu}$. Note that $\mathcal{T}_{\bar{\mu}}$ is a subtree of $\mq$ as well. Recall that $\md^-$ is a path of  $\mq^-$. Let $\md_{\bar{\mu}} = \md^{-} \cap \mathcal{T}_{\bar{\mu}}$ be the subpath of $\md$ in the tree $\mathcal{T}_{\bar{\mu}}$. It is possible that $\md_{\bar{\mu}} = \emptyset$. 
	\begin{claim}\label{clm:Tmu-delta} Let $\Delta(\mt_{\bar{\mu}}) = \Phi(\mt_{\bar{\mu}}) - \adm(\md_{\bar{\nu}})$ where $\Phi(\mt_{\bar{\mu}})  = \sum_{\varphi \in \mv(\mt_{\bar{\mu}})}\omega(\varphi) + \sum_{\mbe \in \msttilde_i\cap \me(\mt_{\bar{\mu}})}w(\mbe)$. Then:
		$$\Delta(\mt_{\bar{\mu}}) = \Omega(| \mv(\mt_{\bar{\mu}})|\epsi L_i).$$
	\end{claim}
	\begin{proof}
		By Item (3) of \Cref{lm:tree-clustering},  $\adm(\mt_{\bar{\mu}} \setminus \md_{\bar{\mu}}) = \Omega( \md_{\bar{\mu}}) = \Omega(|\mv(\md_{\bar{\mu}})|\eps L_i)$. Clearly, $\adm(\mt_{\bar{\mu}} \setminus \md_{\bar{\mu}}) = \Omega(|\mv(\mt_{\bar{\mu}})| - |\mv(\md_{\bar{\mu}})|)\eps L_i$.  Thus, 
		\begin{equation*}
			\begin{split}
				\Delta(\mt_{\bar{\mu}}) &\geq \adm(\mt_{\bar{\mu}} \setminus \md_{\bar{\mu}}) = (\adm(\mt_{\bar{\mu}} \setminus \md_{\bar{\mu}}))/2 +  \adm(\mt_{\bar{\mu}} \setminus \md_{\bar{\mu}})/2\\
				& =  \Omega(|\mv(\mt_{\bar{\mu}})| - |\mv(\md_{\bar{\mu}})|)\eps L_i + \Omega(|\mv(\md_{\bar{\mu}})|\eps L_i)=   \Omega(|\mv(\mt_{\bar{\mu}})|\eps L_i)~,
			\end{split}
		\end{equation*}
		as claimed. \qed
	\end{proof}
	
	Since $\adm(\md)\leq \adm(\md^{-})$, we have:
	\begin{equation*}
		\begin{split}
			\Delta^+_{i+1} (\mq) &\geq  \Phi(\mq) - \adm(\md^{-})  =\Phi(\mq-) - \adm(\md^{-})\\
			& = \sum_{\bar{\mu}\in \Qbar\cap \bar{W}}\Delta(\mt_{\bar{\mu}})  \\
			&=  \sum_{\bar{\mu}\in \Qbar\cap \bar{W}} \Omega(| \mv(\mt_{\bar{\mu}})|\epsi L_i) \qquad \mbox{(by \Cref{clm:Tmu-delta})}\\
			&= \Omega(|\mv(\mq)\cap \tilde{W}|\epsi L_i),
		\end{split}
	\end{equation*}
	Thus, \Cref{eq:blacknodes-C} holds as claimed. \qed
\end{proof}




==> Glossary.tex <==


\section{Glossary for notation used in \Cref{subsec:framework-intro}}


\renewcommand{\arraystretch}{1.3}
\begin{table}[H]
	\begin{longtable}{| l | l|} 
		\hline
		\textbf{Notation} & \textbf{Meaning} \\ \hline
		$t,\eps$ & Stretch parameters, $t\geq 1, \eps \ll 1$.\\ \hline 
		$\nor2{p,q}$ & Euclidean distance between two points $p,q\in \mathbb{R}^d$.\\ \hline 
		$\alpha(m,n)$ &  The inverse Ackermann function.\\ \hline 
		$H_{<L}$ & $t(1+\gamma \eps)$-spanner for edges of weights less than $L$.\\ \hline 
		$\gamma$ & Stretch parameter in  $H_{< L}$;  $\gamma\geq 1$.\\ \hline 
		$L,\beta, \Upsilon$ & %Parameters in $(L,\eps,\beta,\Upsilon)$-cluster graph (\Cref{def:ClusterGraph-Param}\\\hline
		\shortstack{Parameters in $(L,\eps,\beta,\Upsilon)$-cluster graph (\Cref{def:ClusterGraph-Param}); \\  $\Upsilon$ takes two values: $(1+\eps)$ or $1+1/250$.}  \\ \hline 
		$\mg = (\mv,\me,\omega)$ &  The $(L,\eps,\beta,\Upsilon)$-cluster graph;  $L \leq \omega(\varphi_{C_1},\varphi_{C_2}) < \Upsilon L$  $\forall (\varphi_{C_1},\varphi_{C_2})\in \me$. \\ \hline 
		$\varphi_C$ &  The node in $\mg$ corresponding to a cluster $C$.\\ \hline 
		$\ssa$ & The sparse spanner \hyperlink{SPSSA}{algorithm}.\\ \hline 
		$\sso$ & The \hyperlink{SPSSO}{sparse spanner oracle}.\\ \hline 
		$\chi$ & The  sparsity parameter of \hyperlink{SparsitySSA}{$\ssa$} and \hyperlink{SparsitySSO}{$\sso$}.\\ \hline
		$s_{\ssa}(\cdot)$ & The \hyperlink{StretchSSA}{stretch} function of $\ssa$.\\ \hline  
		$s_{\sso}$ & The  \hyperlink{StretchSSO}{stretch} function of $\sso$.\\ \hline 
		$\tau(\cdot, \cdot)$ & The function in the running time of $\ssa$.\\ \hline 
		$F$ &  The set of edges of $G$ returned by $\sso$.\\ \hline 
		$\source(\varphi_{C})$ & This returns the representative $r(C)$ in cluster $C$.\\ \hline 
		$\source(\varphi_{C_1}, \varphi_{C_2})$ & This returns the corresponding edge $(u,v)$ of  $(\varphi_{C_1}, \varphi_{C_2}) \in \me$. \\ \hline 
		$\gsso$ & The general sparse spanner oracle.\\ \hline 
		$\mathcal{O}_{G,t}$ & $\gsso$ of $G$ with stretch $t$.\\ \hline 
		$\wsp_{\mathcal{O}_{G,t}}$ & The weak sparsity of the $\gsso$ $\mathcal{O}_{G,t}$.\\ \hline 
		$\ssp_{\mathcal{O}_{G,t}}$ & The strong sparsity of the $\gsso$ $\mathcal{O}_{G,t}$.\\ \hline 
	\end{longtable}
	\caption{Notation introduced in \Cref{subsec:framework-intro} and used throughout the paper.}
	\label{table:glossray}
\end{table}
\renewcommand{\arraystretch}{1}




==> figs/TheoremProofs.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,456); %set diagram left start at 0, and has height of 456

%Straight Lines [id:da8293467838498436] 
\draw    (122.77,138.33) -- (142.62,138.33) ;
\draw [shift={(120.77,138.33)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw   (191.67,138.33) .. controls (191.67,133.55) and (195.55,129.67) .. (200.33,129.67) .. controls (205.12,129.67) and (209,133.55) .. (209,138.33) .. controls (209,143.12) and (205.12,147) .. (200.33,147) .. controls (195.55,147) and (191.67,143.12) .. (191.67,138.33) -- cycle ; \draw   (196.67,138.33) -- (204,138.33) ; \draw   (200.33,135) -- (200.33,142) ;
\draw   (491.76,138.33) .. controls (491.76,133.55) and (495.64,129.67) .. (500.43,129.67) .. controls (505.22,129.67) and (509.1,133.55) .. (509.1,138.33) .. controls (509.1,143.12) and (505.22,147) .. (500.43,147) .. controls (495.64,147) and (491.76,143.12) .. (491.76,138.33) -- cycle ; \draw   (496.76,138.33) -- (504.1,138.33) ; \draw   (500.43,135) -- (500.43,142) ;
\draw   (541.67,138.33) .. controls (541.67,133.55) and (545.55,129.67) .. (550.33,129.67) .. controls (555.12,129.67) and (559,133.55) .. (559,138.33) .. controls (559,143.12) and (555.12,147) .. (550.33,147) .. controls (545.55,147) and (541.67,143.12) .. (541.67,138.33) -- cycle ; \draw   (546,138.33) -- (554,138.33) ; \draw   (550.33,135) -- (550.33,142) ;
%Straight Lines [id:da12859475684608013] 
\draw    (209.17,138.33) -- (229.02,138.33) ;
\draw [shift={(231.02,138.33)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9993287837921137] 
\draw    (473.67,138.33) -- (492.19,138.33) ;
\draw [shift={(471.67,138.33)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8819240453543753] 
\draw    (559.6,138.33) -- (579.45,138.33) ;
\draw [shift={(581.45,138.33)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da7785191774328355] 
\draw    (151,80.23) -- (151,127.34) ;
\draw [shift={(151,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4191372593174387] 
\draw    (151,80.23) -- (551,80.23) ;
%Straight Lines [id:da41504007096264806] 
\draw    (500.43,80.23) -- (500.43,127.34) ;
\draw [shift={(500.43,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da005041232675436547] 
\draw    (551,80.23) -- (551,127.34) ;
\draw [shift={(551,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4264042425801904] 
\draw    (200.25,80.48) -- (200.25,127.59) ;
\draw [shift={(200.25,129.59)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8542522085244955] 
\draw    (351.17,59.33) -- (351,80.23) ;
%Straight Lines [id:da3781959918557467] 
\draw    (150.07,138.33) ;
\draw   (142.27,138.33) .. controls (142.27,133.55) and (146.15,129.67) .. (150.93,129.67) .. controls (155.72,129.67) and (159.6,133.55) .. (159.6,138.33) .. controls (159.6,143.12) and (155.72,147) .. (150.93,147) .. controls (146.15,147) and (142.27,143.12) .. (142.27,138.33) -- cycle ; \draw   (147,138.33) -- (154.6,138.33) ; \draw   (150.93,135) -- (150.93,142) ;
%Straight Lines [id:da7779497272854068] 
\draw    (120.5,207.34) -- (151,207.34) ;
%Straight Lines [id:da4400517576455787] 
\draw    (151,148.09) -- (151,207.34) ;
\draw [shift={(151,146.09)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da02653692567798971] 
\draw    (200.25,148.59) -- (200.25,207.84) ;
\draw [shift={(200.25,146.59)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6484801551256596] 
\draw    (200.25,207.84) -- (230.75,207.84) ;
%Straight Lines [id:da49844979941595113] 
\draw    (469.75,205.72) -- (500.25,205.72) ;
%Straight Lines [id:da779897098725179] 
\draw    (500.25,148.59) -- (500.25,205.72) ;
\draw [shift={(500.25,146.59)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da19742071313786402] 
\draw    (550.25,148.84) -- (550.25,205.97) ;
\draw [shift={(550.25,146.84)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da024558628814087102] 
\draw    (550.25,205.97) -- (580.75,205.97) ;
\draw   (47.6,254.7) .. controls (47.6,249.91) and (51.48,246.03) .. (56.27,246.03) .. controls (61.05,246.03) and (64.93,249.91) .. (64.93,254.7) .. controls (64.93,259.48) and (61.05,263.36) .. (56.27,263.36) .. controls (51.48,263.36) and (47.6,259.48) .. (47.6,254.7) -- cycle ; \draw   (53,254.7) -- (59.93,254.7) ; \draw   (56.27,251.03) -- (56.27,258.36) ;
\draw   (275.6,254.7) .. controls (275.6,249.91) and (279.48,246.03) .. (284.27,246.03) .. controls (289.05,246.03) and (292.93,249.91) .. (292.93,254.7) .. controls (292.93,259.48) and (289.05,263.36) .. (284.27,263.36) .. controls (279.48,263.36) and (275.6,259.48) .. (275.6,254.7) -- cycle ; \draw   (280.6,254.7) -- (287.93,254.7) ; \draw   (284.27,251.03) -- (284.27,258.36) ;
\draw   (406.93,254.7) .. controls (406.93,249.91) and (410.81,246.03) .. (415.6,246.03) .. controls (420.39,246.03) and (424.27,249.91) .. (424.27,254.7) .. controls (424.27,259.48) and (420.39,263.36) .. (415.6,263.36) .. controls (410.81,263.36) and (406.93,259.48) .. (406.93,254.7) -- cycle ; \draw   (411.93,254.7) -- (419.27,254.7) ; \draw   (415.6,251.03) -- (415.6,258.36) ;
%Straight Lines [id:da2720756344987463] 
\draw    (56.17,265.74) -- (56.17,327.83) ;
\draw [shift={(56.17,263.74)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da921043892768213] 
\draw    (56.17,327.83) -- (258.71,327.83) ;
%Straight Lines [id:da7929041663623573] 
\draw    (445.5,327.83) -- (646.8,327.83) ;
\draw   (638.27,254.7) .. controls (638.27,249.91) and (642.15,246.03) .. (646.93,246.03) .. controls (651.72,246.03) and (655.6,249.91) .. (655.6,254.7) .. controls (655.6,259.48) and (651.72,263.36) .. (646.93,263.36) .. controls (642.15,263.36) and (638.27,259.48) .. (638.27,254.7) -- cycle ; \draw   (643.27,254.7) -- (651,254.7) ; \draw   (646.93,251.03) -- (646.93,258.36) ;
%Straight Lines [id:da32594437558444445] 
\draw    (646.8,265.74) -- (646.8,327.83) ;
\draw [shift={(646.8,263.74)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9155506945034109] 
\draw    (56.26,223.57) -- (56.26,245.57) ;
\draw [shift={(56.26,221.57)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da00525714250057141] 
\draw    (284.22,223.79) -- (284.22,245.79) ;
\draw [shift={(284.22,221.79)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9530405404433144] 
\draw    (415.56,223.57) -- (415.56,245.57) ;
\draw [shift={(415.56,221.57)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6542015909128751] 
\draw    (646.89,223.57) -- (646.89,245.57) ;
\draw [shift={(646.89,221.57)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9424305848934773] 
\draw    (94.45,254.48) -- (66.81,254.48) ;
\draw [shift={(64.81,254.48)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6468046720334764] 
\draw    (308.09,254.62) -- (295,254.62) ;
\draw [shift={(293,254.62)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da682726931389859] 
\draw    (426.27,254.62) -- (441.55,254.62) ;
\draw [shift={(424.27,254.62)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da35326306206125624] 
\draw    (617.77,254.81) -- (636.27,254.81) ;
\draw [shift={(638.27,254.81)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9806269672627577] 
\draw    (284.3,265.34) -- (284.3,301.71) ;
\draw [shift={(284.3,263.34)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da366086198166405] 
\draw    (415.58,265.16) -- (415.58,301.53) ;
\draw [shift={(415.58,263.16)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;

% Text Node
\draw    (289.67,7.83) -- (412.67,7.83) -- (412.67,59.83) -- (289.67,59.83) -- cycle  ;
\draw (351.17,33.83) node   [align=left] {\begin{minipage}[lt]{80.69pt}\setlength\topsep{0pt}
\begin{center}
Lemma 1.5\\unified framework
\end{center}

\end{minipage}};
% Text Node
\draw    (11.81,113.83) -- (120.81,113.83) -- (120.81,162.83) -- (11.81,162.83) -- cycle  ;
\draw (66.31,138.33) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
Theorem 1.1\\ACT Euclidean
\end{center}

\end{minipage}};
% Text Node
\draw    (231.45,113.33) -- (340.45,113.33) -- (340.45,163.33) -- (231.45,163.33) -- cycle  ;
\draw (285.95,138.33) node   [align=left] {\begin{minipage}[lt]{71.24pt}\setlength\topsep{0pt}
\begin{center}
Lemma 1.5\\General Graphs
\end{center}

\end{minipage}};
% Text Node
\draw    (361.67,113.83) -- (470.67,113.83) -- (470.67,162.83) -- (361.67,162.83) -- cycle  ;
\draw (416.17,138.33) node   [align=left] {\begin{minipage}[lt]{71.3pt}\setlength\topsep{0pt}
\begin{center}
Lemma 1.5\\Unit Disk
\end{center}

\end{minipage}};
% Text Node
\draw    (581.76,113.83) -- (690.76,113.83) -- (690.76,162.83) -- (581.76,162.83) -- cycle  ;
\draw (636.26,138.33) node   [align=left] {\begin{minipage}[lt]{71.52pt}\setlength\topsep{0pt}
\begin{center}
Lemma 1.5\\Minor-Free
\end{center}

\end{minipage}};
% Text Node
\draw    (258.5,301.83) -- (445.5,301.83) -- (445.5,353.83) -- (258.5,353.83) -- cycle  ;
\draw (352,327.83) node   [align=left] {\begin{minipage}[lt]{124.67pt}\setlength\topsep{0pt}
\begin{center}
Lemma 3.21\\Algorithm $\mathcal{A}$
\end{center}

\end{minipage}};
% Text Node
\draw    (11.38,191.39) -- (120.38,191.39) -- (120.38,221.39) -- (11.38,221.39) -- cycle  ;
\draw (65.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
Theorem 1.6
\end{center}

\end{minipage}};
% Text Node
\draw    (231.38,191.39) -- (340.38,191.39) -- (340.38,221.39) -- (231.38,221.39) -- cycle  ;
\draw (285.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
Theorem 1.7
\end{center}

\end{minipage}};
% Text Node
\draw    (361.38,191.39) -- (470.38,191.39) -- (470.38,221.39) -- (361.38,221.39) -- cycle  ;
\draw (415.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
Theorem 1.8
\end{center}

\end{minipage}};
% Text Node
\draw    (581.38,191.39) -- (690.38,191.39) -- (690.38,221.39) -- (581.38,221.39) -- cycle  ;
\draw (635.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
Theorem 1.9
\end{center}

\end{minipage}};
% Text Node
\draw    (94.31,233.7) -- (180.31,233.7) -- (180.31,275.7) -- (94.31,275.7) -- cycle  ;
\draw (137.31,254.7) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
Lemma 4.1\\A$\mathbb{R}^d$
\end{center}

\end{minipage}};
% Text Node
\draw    (441.78,233.7) -- (527.78,233.7) -- (527.78,275.7) -- (441.78,275.7) -- cycle  ;
\draw (484.78,254.7) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
Lemma 4.1\\$A\mathbb{R}^d$
\end{center}

\end{minipage}};
% Text Node
\draw    (308.17,233.7) -- (394.17,233.7) -- (394.17,275.7) -- (308.17,275.7) -- cycle  ;
\draw (351.17,254.7) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
Lemma 4.2\\$A_G$
\end{center}

\end{minipage}};
% Text Node
\draw    (532.7,234.08) -- (617.7,234.08) -- (617.7,275.08) -- (532.7,275.08) -- cycle  ;
\draw (575.2,254.58) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
Lemma 4.3\\$A_{Kr}$
\end{center}

\end{minipage}};


\end{tikzpicture}

==> figs/TheoremProofs2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,456); %set diagram left start at 0, and has height of 456

%Straight Lines [id:da8293467838498436] 
\draw    (122.77,138.33) -- (142.62,138.33) ;
\draw [shift={(120.77,138.33)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw   (191.67,138.33) .. controls (191.67,133.55) and (195.55,129.67) .. (200.33,129.67) .. controls (205.12,129.67) and (209,133.55) .. (209,138.33) .. controls (209,143.12) and (205.12,147) .. (200.33,147) .. controls (195.55,147) and (191.67,143.12) .. (191.67,138.33) -- cycle ; \draw   (191.67,138.33) -- (209,138.33) ; \draw   (200.33,129.67) -- (200.33,147) ;
\draw   (491.76,138.33) .. controls (491.76,133.55) and (495.64,129.67) .. (500.43,129.67) .. controls (505.22,129.67) and (509.1,133.55) .. (509.1,138.33) .. controls (509.1,143.12) and (505.22,147) .. (500.43,147) .. controls (495.64,147) and (491.76,143.12) .. (491.76,138.33) -- cycle ; \draw   (491.76,138.33) -- (509.1,138.33) ; \draw   (500.43,129.67) -- (500.43,147) ;
\draw   (541.67,138.33) .. controls (541.67,133.55) and (545.55,129.67) .. (550.33,129.67) .. controls (555.12,129.67) and (559,133.55) .. (559,138.33) .. controls (559,143.12) and (555.12,147) .. (550.33,147) .. controls (545.55,147) and (541.67,143.12) .. (541.67,138.33) -- cycle ; \draw   (541.67,138.33) -- (559,138.33) ; \draw   (550.33,129.67) -- (550.33,147) ;
%Straight Lines [id:da12859475684608013] 
\draw    (209.17,138.33) -- (229.02,138.33) ;
\draw [shift={(231.02,138.33)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9993287837921137] 
\draw    (473.67,138.33) -- (492.19,138.33) ;
\draw [shift={(471.67,138.33)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8819240453543753] 
\draw    (559.6,138.33) -- (579.45,138.33) ;
\draw [shift={(581.45,138.33)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da7785191774328355] 
\draw    (151,80.23) -- (151,127.34) ;
\draw [shift={(151,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4191372593174387] 
\draw    (151,80.23) -- (551,80.23) ;
%Straight Lines [id:da41504007096264806] 
\draw    (500.43,80.23) -- (500.43,127.34) ;
\draw [shift={(500.43,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da005041232675436547] 
\draw    (551,80.23) -- (551,127.34) ;
\draw [shift={(551,129.34)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4264042425801904] 
\draw    (200.25,80.48) -- (200.25,127.59) ;
\draw [shift={(200.25,129.59)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8542522085244955] 
\draw    (351.17,59.33) -- (351,80.23) ;
%Straight Lines [id:da3781959918557467] 
\draw    (150.07,138.33) ;
\draw   (142.27,138.33) .. controls (142.27,133.55) and (146.15,129.67) .. (150.93,129.67) .. controls (155.72,129.67) and (159.6,133.55) .. (159.6,138.33) .. controls (159.6,143.12) and (155.72,147) .. (150.93,147) .. controls (146.15,147) and (142.27,143.12) .. (142.27,138.33) -- cycle ; \draw   (142.27,138.33) -- (159.6,138.33) ; \draw   (150.93,129.67) -- (150.93,147) ;
%Straight Lines [id:da4400517576455787] 
\draw    (151,148.09) -- (151,190.32) ;
\draw [shift={(151,146.09)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da02653692567798971] 
\draw    (200.25,148.45) -- (200.25,190.68) ;
\draw [shift={(200.25,146.45)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da49844979941595113] 
\draw    (469.75,205.72) -- (500.25,205.72) ;
%Straight Lines [id:da779897098725179] 
\draw    (500.25,148.59) -- (500.25,205.72) ;
\draw [shift={(500.25,146.59)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da19742071313786402] 
\draw    (550.25,148.84) -- (550.25,205.97) ;
\draw [shift={(550.25,146.84)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da024558628814087102] 
\draw    (550.25,205.97) -- (580.75,205.97) ;
\draw   (166.68,263.2) .. controls (166.68,258.41) and (170.56,254.53) .. (175.35,254.53) .. controls (180.14,254.53) and (184.02,258.41) .. (184.02,263.2) .. controls (184.02,267.98) and (180.14,271.86) .. (175.35,271.86) .. controls (170.56,271.86) and (166.68,267.98) .. (166.68,263.2) -- cycle ; \draw   (166.68,263.2) -- (184.02,263.2) ; \draw   (175.35,254.53) -- (175.35,271.86) ;
%Straight Lines [id:da921043892768213] 
\draw    (175.33,327.83) -- (258.71,327.83) ;
%Straight Lines [id:da7929041663623573] 
\draw    (445.5,327.83) -- (636,327.83) ;
%Straight Lines [id:da4153329362550173] 
\draw    (175.33,223.01) -- (175.33,254.84) ;
\draw [shift={(175.33,221.01)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da08151713511199477] 
\draw    (125,263.2) -- (164.5,263.2) ;
\draw [shift={(166.5,263.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw   (406.68,263.2) .. controls (406.68,258.41) and (410.56,254.53) .. (415.35,254.53) .. controls (420.14,254.53) and (424.02,258.41) .. (424.02,263.2) .. controls (424.02,267.98) and (420.14,271.86) .. (415.35,271.86) .. controls (410.56,271.86) and (406.68,267.98) .. (406.68,263.2) -- cycle ; \draw   (406.68,263.2) -- (424.02,263.2) ; \draw   (415.35,254.53) -- (415.35,271.86) ;
%Straight Lines [id:da9458895500155264] 
\draw    (415.33,224.01) -- (415.33,254.51) ;
\draw [shift={(415.33,222.01)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4673311657670407] 
\draw    (365,263.2) -- (404.5,263.2) ;
\draw [shift={(406.5,263.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw   (627.68,263.2) .. controls (627.68,258.41) and (631.56,254.53) .. (636.35,254.53) .. controls (641.14,254.53) and (645.02,258.41) .. (645.02,263.2) .. controls (645.02,267.98) and (641.14,271.86) .. (636.35,271.86) .. controls (631.56,271.86) and (627.68,267.98) .. (627.68,263.2) -- cycle ; \draw   (627.68,263.2) -- (645.02,263.2) ; \draw   (636.35,254.53) -- (636.35,271.86) ;
%Straight Lines [id:da9846230198940495] 
\draw    (636.33,224.01) -- (636.33,254.51) ;
\draw [shift={(636.33,222.01)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da09799274050553963] 
\draw    (586,263.2) -- (625.5,263.2) ;
\draw [shift={(627.5,263.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da10943990039983897] 
\draw    (175.33,271.34) -- (175.33,327.83) ;
%Straight Lines [id:da4466330394081508] 
\draw    (636,271.34) -- (636,327.84) ;
%Straight Lines [id:da3147396855879727] 
\draw    (415.44,271.78) -- (415.44,301.62) ;

% Text Node
\draw    (289.67,7.83) -- (412.67,7.83) -- (412.67,59.83) -- (289.67,59.83) -- cycle  ;
\draw (351.17,33.83) node   [align=left] {\begin{minipage}[lt]{80.69pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:framework}\\unified framework
\end{center}

\end{minipage}};
% Text Node
\draw    (11.81,113.83) -- (120.81,113.83) -- (120.81,162.83) -- (11.81,162.83) -- cycle  ;
\draw (66.31,138.33) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:ACT}\\ACT Euclidean
\end{center}

\end{minipage}};
% Text Node
\draw    (231.45,113.33) -- (340.45,113.33) -- (340.45,163.33) -- (231.45,163.33) -- cycle  ;
\draw (285.95,138.33) node   [align=left] {\begin{minipage}[lt]{71.24pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:UDG-fast}\\Unit Disk
\end{center}

\end{minipage}};
% Text Node
\draw    (361.67,113.83) -- (470.67,113.83) -- (470.67,162.83) -- (361.67,162.83) -- cycle  ;
\draw (416.17,138.33) node   [align=left] {\begin{minipage}[lt]{71.3pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:general-fast}\\General Graphs
\end{center}

\end{minipage}};
% Text Node
\draw    (581.76,113.83) -- (690.76,113.83) -- (690.76,162.83) -- (581.76,162.83) -- cycle  ;
\draw (636.26,138.33) node   [align=left] {\begin{minipage}[lt]{71.52pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:minor-free-fast}\\Minor-Free
\end{center}

\end{minipage}};
% Text Node
\draw    (258.5,301.83) -- (445.5,301.83) -- (445.5,353.83) -- (258.5,353.83) -- cycle  ;
\draw (352,327.83) node   [align=left] {\begin{minipage}[lt]{124.67pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:ConstructH_i}\\Algorithm $\mathcal{A}$
\end{center}

\end{minipage}};
% Text Node
\draw    (120.72,191.39) -- (229.72,191.39) -- (229.72,221.39) -- (120.72,221.39) -- cycle  ;
\draw (175.22,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:ACTUDGClustering}
\end{center}

\end{minipage}};
% Text Node
\draw    (361.38,191.39) -- (470.38,191.39) -- (470.38,221.39) -- (361.38,221.39) -- cycle  ;
\draw (415.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:GeneralClustering}
\end{center}

\end{minipage}};
% Text Node
\draw    (581.38,191.39) -- (690.38,191.39) -- (690.38,221.39) -- (581.38,221.39) -- cycle  ;
\draw (635.88,206.39) node   [align=left] {\begin{minipage}[lt]{71.66pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:MinorClustering}
\end{center}

\end{minipage}};
% Text Node
\draw    (39.56,242.7) -- (124.56,242.7) -- (124.56,283.7) -- (39.56,283.7) -- cycle  ;
\draw (82.06,263.2) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:ACT-UDG}\\$\ma_{\geom}$
\end{center}

\end{minipage}};
% Text Node
\draw    (279.56,242.7) -- (364.56,242.7) -- (364.56,283.7) -- (279.56,283.7) -- cycle  ;
\draw (322.06,263.2) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:App-Gen}\\$\ma_{\gen}$
\end{center}

\end{minipage}};
% Text Node
\draw    (500.56,242.7) -- (585.56,242.7) -- (585.56,283.7) -- (500.56,283.7) -- cycle  ;
\draw (543.06,263.2) node   [align=left] {\begin{minipage}[lt]{55.17pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:App-Minor}\\$\ma_{\minor}$
\end{center}

\end{minipage}};


\end{tikzpicture}


==> figs/Unified2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,748); %set diagram left start at 0, and has height of 748
	
	%Straight Lines [id:da43353968645182106] 
	\draw    (160,69.33) -- (160,204.67) -- (159,426) -- (159,662.84) ;
	%Straight Lines [id:da550947224938801] 
	\draw    (159.57,129.95) -- (127.24,129.95) ;
	\draw [shift={(125.24,129.95)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	%Straight Lines [id:da8018925595960429] 
	\draw    (159,309.9) -- (127.67,309.9) ;
	\draw [shift={(125.67,309.9)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	%Straight Lines [id:da9707593108875174] 
	\draw    (158,484.9) -- (126.67,484.9) ;
	\draw [shift={(124.67,484.9)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	%Straight Lines [id:da21168349357779248] 
	\draw    (159,662.84) -- (127.67,662.84) ;
	\draw [shift={(125.67,662.84)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	
	
	% Text Node
	\draw    (109.67,14.83) -- (266.67,14.83) -- (266.67,68.83) -- (109.67,68.83) -- cycle  ;
	\draw (188.17,41.83) node   [align=left] {\begin{minipage}[lt]{104.04pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{lm:framework}\\Unified Framework
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw (175.5,297.5) node [anchor=north west][inner sep=0.75pt]  [rotate=-90] [align=left] {\textsc{Fast Construction}};
	\draw    (7.25,93.86) -- (124.25,93.86) -- (124.25,166.86) -- (7.25,166.86) -- cycle  ;
	\draw (65.75,130.36) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:ACT}\\Fast ACT\\Euclidean
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw    (7.25,217.44) -- (124.25,217.44) -- (124.25,246.44) -- (7.25,246.44) -- cycle  ;
	\draw (65.75,231.94) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:ACTUDGClustering}
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw (28.25,200.34) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
	% Text Node
	\draw    (7.25,273.36) -- (124.25,273.36) -- (124.25,346.36) -- (7.25,346.36) -- cycle  ;
	\draw (65.75,309.86) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:UDG-fast}\\Fast Spanners\\ UDG
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw    (7.25,392.99) -- (124.25,392.99) -- (124.25,421.99) -- (7.25,421.99) -- cycle  ;
	\draw (65.75,407.49) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:GeneralClustering}
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw (28.25,375.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
	% Text Node
	\draw    (7.25,448.9) -- (124.25,448.9) -- (124.25,521.9) -- (7.25,521.9) -- cycle  ;
	\draw (65.75,485.4) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:general-fast}\\Fast Spanners\\General Graphs
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw    (8.25,569.99) -- (125.25,569.99) -- (125.25,598.99) -- (8.25,598.99) -- cycle  ;
	\draw (66.75,584.49) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:MinorClustering}
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw (29.25,552.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
	% Text Node
	\draw    (8.25,625.9) -- (125.25,625.9) -- (125.25,698.9) -- (8.25,698.9) -- cycle  ;
	\draw (66.75,662.4) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
			\begin{center}
				\Cref{thm:minor-free-fast}\\Fast Spanner\\Minor-free
			\end{center}
	\end{minipage}};
	% Connection
	\draw    (65.75,246.44) -- (65.75,271.36) ;
	\draw [shift={(65.75,273.36)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	% Connection
	\draw    (65.75,196.34) -- (65.75,168.86) ;
	\draw [shift={(65.75,166.86)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	% Connection
	\draw    (65.75,421.99) -- (65.75,446.9) ;
	\draw [shift={(65.75,448.9)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	% Connection
	\draw    (66.75,598.99) -- (66.75,623.9) ;
	\draw [shift={(66.75,625.9)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
	
\end{tikzpicture}


==> figs/Unified3.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,748); %set diagram left start at 0, and has height of 748

%Straight Lines [id:da43353968645182106] 
\draw    (160,69.33) -- (160,204.67) -- (159,426) -- (159,662.84) ;
%Straight Lines [id:da550947224938801] 
\draw    (159.57,129.95) -- (127.24,129.95) ;
\draw [shift={(125.24,129.95)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8018925595960429] 
\draw    (159,309.9) -- (127.67,309.9) ;
\draw [shift={(125.67,309.9)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8453570835526145] 
\draw    (216.67,69.33) -- (216.67,191.83) -- (216.67,354.5) -- (216.67,663.09) ;
%Shape: Rectangle [id:dp32803694517951243] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.11 ][dash pattern={on 4.5pt off 4.5pt}] (187.67,80) -- (397.67,80) -- (397.67,733) -- (187.67,733) -- cycle ;
%Straight Lines [id:da9707593108875174] 
\draw    (158,484.9) -- (126.67,484.9) ;
\draw [shift={(124.67,484.9)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da21168349357779248] 
\draw    (159,662.84) -- (127.67,662.84) ;
\draw [shift={(125.67,662.84)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da21991952545049465] 
\draw    (249,130.58) -- (216.67,130.58) ;
\draw [shift={(251,130.58)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da3441870057449532] 
\draw    (249,263.71) -- (216.67,263.71) ;
\draw [shift={(251,263.71)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da29957355564081656] 
\draw    (250,396.84) -- (217.67,396.84) ;
\draw [shift={(252,396.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6629840865542558] 
\draw    (249,663.09) -- (216.67,663.09) ;
\draw [shift={(251,663.09)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da02027266410290096] 
\draw    (248.5,529.97) -- (216.17,529.97) ;
\draw [shift={(250.5,529.97)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;

% Text Node
\draw    (109.67,14.83) -- (266.67,14.83) -- (266.67,68.83) -- (109.67,68.83) -- cycle  ;
\draw (188.17,41.83) node   [align=left] {\begin{minipage}[lt]{104.04pt}\setlength\topsep{0pt}
\begin{center}
\Cref{lm:framework}\\Unified Framework
\end{center}

\end{minipage}};
% Text Node
\draw (175.5,297.5) node [anchor=north west][inner sep=0.75pt]  [rotate=-90] [align=left] {\textsc{Fast Construction}};
% Text Node
\draw (197.5,418) node [anchor=north west][inner sep=0.75pt]  [rotate=-270] [align=left] {\textsc{Optimal Lightness}};
% Text Node
\draw    (7.25,93.86) -- (124.25,93.86) -- (124.25,166.86) -- (7.25,166.86) -- cycle  ;
\draw (65.75,130.36) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
 \Cref{thm:ACT}\\Fast ACT\\Euclidean
\end{center}

\end{minipage}};
% Text Node
\draw    (7.25,217.44) -- (124.25,217.44) -- (124.25,246.44) -- (7.25,246.44) -- cycle  ;
\draw (65.75,231.94) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:ACTUDGClustering}
\end{center}

\end{minipage}};
% Text Node
\draw (28.25,200.34) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
% Text Node
\draw    (7.25,273.36) -- (124.25,273.36) -- (124.25,346.36) -- (7.25,346.36) -- cycle  ;
\draw (65.75,309.86) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:UDG-fast}\\Fast Spanners\\ UDG
\end{center}

\end{minipage}};
% Text Node
\draw    (7.25,392.99) -- (124.25,392.99) -- (124.25,421.99) -- (7.25,421.99) -- cycle  ;
\draw (65.75,407.49) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:GeneralClustering}
\end{center}

\end{minipage}};
% Text Node
\draw (28.25,375.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
% Text Node
\draw    (7.25,448.9) -- (124.25,448.9) -- (124.25,521.9) -- (7.25,521.9) -- cycle  ;
\draw (65.75,485.4) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:general-fast}\\Fast Spanners\\General Graphs
\end{center}

\end{minipage}};
% Text Node
\draw    (8.25,569.99) -- (125.25,569.99) -- (125.25,598.99) -- (8.25,598.99) -- cycle  ;
\draw (66.75,584.49) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:MinorClustering}
\end{center}

\end{minipage}};
% Text Node
\draw (29.25,552.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {(\Cref{sec:applications})};
% Text Node
\draw    (8.25,625.9) -- (125.25,625.9) -- (125.25,698.9) -- (8.25,698.9) -- cycle  ;
\draw (66.75,662.4) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
\Cref{thm:minor-free-fast}\\Fast Spanner\\Minor-free
\end{center}

\end{minipage}};
% Text Node
\draw    (251.08,93.36) -- (369.08,93.36) -- (369.08,167.36) -- (251.08,167.36) -- cycle  ;
\draw (310.08,130.36) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
Optimal \\Light Spanners\\General Graphs
\end{center}

\end{minipage}};
% Text Node
\draw    (251.08,229.03) -- (369.08,229.03) -- (369.08,303.03) -- (251.08,303.03) -- cycle  ;
\draw (310.08,266.03) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
Optimal\\ Light Euclidean \\ Spanners
\end{center}

\end{minipage}};
% Text Node
\draw    (251.08,360.36) -- (369.08,360.36) -- (369.08,434.36) -- (251.08,434.36) -- cycle  ;
\draw (310.08,397.36) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
Light Spanners\\Normed Spaces
\end{center}

\end{minipage}};
% Text Node
\draw    (251.08,492.03) -- (369.08,492.03) -- (369.08,566.03) -- (251.08,566.03) -- cycle  ;
\draw (310.08,529.03) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
Optimal \\Light Spanners\\Minor-free
\end{center}

\end{minipage}};
% Text Node
\draw    (251.08,626.36) -- (369.08,626.36) -- (369.08,700.36) -- (251.08,700.36) -- cycle  ;
\draw (310.08,663.36) node   [align=left] {\begin{minipage}[lt]{76.97pt}\setlength\topsep{0pt}
\begin{center}
Optimal\\Light Steiner\\Euclidean Spanners
\end{center}

\end{minipage}};
% Connection
\draw    (65.75,246.44) -- (65.75,271.36) ;
\draw [shift={(65.75,273.36)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
% Connection
\draw    (65.75,196.34) -- (65.75,168.86) ;
\draw [shift={(65.75,166.86)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
% Connection
\draw    (65.75,421.99) -- (65.75,446.9) ;
\draw [shift={(65.75,448.9)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
% Connection
\draw    (66.75,598.99) -- (66.75,623.9) ;
\draw [shift={(66.75,625.9)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;

\end{tikzpicture}

